A trust region-type normal map-based semismooth Newton method for nonsmooth nonconvex composite optimization

We propose a novel trust region method for solving a class of nonsmooth, nonconvex composite-type optimization problems. The approach embeds inexact semismooth Newton steps for finding zeros of a normal map-based stationarity measure for the problem in a trust region framework. Based on a new merit function and acceptance mechanism, global convergence and transition to fast local q-superlinear convergence are established under standard conditions. In addition, we verify that the proposed trust region globalization is compatible with the Kurdyka-{\L}ojasiewicz inequality yielding finer convergence results. We further derive new normal map-based representations of the associated second-order optimality conditions that have direct connections to the local assumptions required for fast convergence. Finally, we study the behavior of our algorithm when the Hessian matrix of the smooth part of the objective function is approximated by BFGS updates. We successfully link the KL theory, properties of the BFGS approximations, and a Dennis-Mor{\'e}-type condition to show superlinear convergence of the quasi-Newton version of our method. Numerical experiments on sparse logistic regression, image compression, and a constrained log-determinant problem illustrate the efficiency of the proposed algorithm.

==> decomp.tex <==
\section{Decomposable functions} \label{section:soc:decomp}
%
In the following section, we will introduce and discuss an important class of nonsmooth functions for which the curvature term $\Upsilon(h) = \mathrm{d}^2\vp(\bar x|-\nabla f(\bar x))(h)$ in the second-order condition \cref{eq:soc-org} has a simple representation and is a generalized quadratic as required in assumption \ref{E2}. 

The concept of decomposable functions was proposed by Shapiro in \cite{Sha03} and is strongly related to the notions of amenable functions, see, e.g., \cite{PolRoc92,PolRoc93} or \cite[Chapter 10.F]{RocWet98}, and of $C^{\ell}$-cone reducible sets in nonlinear, constrained optimization. 

We will see that the class of decomposable functions is quite rich and a large number of nonsmooth optimization problems can be treated within the framework of decomposable function. In particular, we will show that $\ell_1$- and group sparse problems possess a decomposable structure. Moreover, decomposability is also applicable to structural more advanced problems such as semidefinite programming or nuclear norm regularized optimization problems. 

In the next paragraph, based on \cite[Definition 1.1]{Sha03}, we give a definition of decomposable functions. Since the framework in \cite{Sha03} is tailored to the real valued setting, we have to adjust the definitions given in \cite{Sha03} to cope with the possible extended valued situation.  Moreover, we also extend the definition in \cite{Sha03} and introduce fully decomposable functions, which will play an essential role in our further analysis.
 
Thereafter, we discuss the main properties of decomposable functions, present various illustrating examples and provide several calculation rules. We conclude this section with one of our main results. 

\subsection{Decomposability}

Let us start with a detailed definition of decomposable functions. 

\begin{definition}[Decomposable functions] \label{definition:soc:decomp-func} A function $\vp:\Rn \to \Rex$ is called $C^\ell$-{decomposable}, $\ell \in \N$, at a point $\bar x \in \dom{\vp}$, if there exists an open neighborhood $U$ of $\bar x$ such that
%
\be \label{eq:soc:decomp-eq} \vp(x) = \vp(\bar x) + \vp_d(F(x)), \quad \forall~x \in U, \ee
%
and the functions $\vp_d$ and $F$ satisfy:
\begin{itemize}
\item[\rmn{(i)}] $F: \Rn \to \Rm$ is $\ell$-times continuously differentiable on $U$ and it holds $F(\bar x) = 0$.
\item[\rmn{(ii)}] The mapping $\vp_d : \Rm \to \Rex$ is convex, proper, lower semicontinuous, and positively homogeneous.
\item[\rmn{(iii)}] Robinson's constraint qualification holds at $\bar x$:
\end{itemize} \vspace{-1.5ex}
\be \label{eq:soc:rob-cq-misc1} 0 \in \inter \{ F(\bar x) + DF(\bar x) \Rn - \dom~\vp_d \} = \inter \{ DF(\bar x) \Rn - \dom~\vp_d \}. \ee
%\end{itemize}
We say that $\vp$ is $C^\ell$-{fully decomposable} at $\bar x$ if $\vp$ is $C^\ell$-decomposable at $\bar x$ and if, in addition, the nondegeneracy condition 
%
\[ DF(\bar x) \Rn + \lin~N_{\partial \vp_d(0)}(\lambda) = \Rm \]
%
is satisfied at $\bar x$ for an arbitrary subgradient $\lambda \in \partial\vp_d(0)$. %Finally, the function $\vp$ is called $C^\ell$-{\rm cone decomposable} at $\bar x$ if $\vp$ is $C^\ell$-fully decomposable at $\bar x$ and the normal cone $N_{\partial \vp_d(0)}(\lambda)$ is pointed, i.e., we have $\lin~N_{\partial \vp_d(0)}(\lambda) = \{0\}$.
\end{definition}

If $\vp$ is decomposable at $\bar x$, then the functions $\vp_d: \Rm \to \Rex$ and $F : \Rn \to \Rm$ are called a {decomposition pair} of $\vp$. Of course, a decomposition of $\vp$ as in \eqref{eq:soc:decomp-eq} does not need to be unique. Thus, in general, the function $\vp$ can have many different decomposition pairs. Let us also mention that, in the fully decomposable case, since the nondegeneracy condition implies Robinson's constraint qualification \eqref{eq:soc:rob-cq-misc1}, assumption (iii) in Definition \ref{definition:soc:decomp-func} is superfluous.  
%Let us also note that cone decomposability implies that the derivative mapping $DF(\bar x) : \Rn \to \Rm$ is onto. 
We continue with two important remarks. 

\begin{remark} \label{remark:soc:rob-decomp} Due to Lemma \ref{lemma:pre:subdiff-homo}, the function $\vp_d$ is subdifferentiable at $0$. Hence, the nondegeneracy condition in Definition \ref{definition:soc:decomp-func} is always well-defined. Moreover, since $\vp_d$ is convex, proper, and positively homogeneous, the set $DF(\bar x)\Rn - \dom~\vp_d$ is a convex, nonempty cone and, consequently, Robinson's constraint qualification \eqref{eq:soc:rob-cq-misc1} is equivalent to the condition
%
 \[ DF(\bar x) \Rn - \dom~\vp_d = \Rm. \] 
%Alternative characterization of the normal cone. Convexity of $\vp_d$! 
\end{remark}

\begin{remark}[Stationarity and decomposable optimization problems] \label{remark:soc:mega} So far, we have only considered the trivial decomposition $F \equiv I$. For more general decompositions as in Definition \ref{definition:soc:decomp-func}, we have to be more careful when speaking of local solutions and stationary points. If the function $\vp$ can be rewritten as a composition $\vp \equiv \vp_d \circ F$, then it is clear that every local solution of the initial problem
\be \label{eq:soc:prob-misc5} \min_x~f(x) + \vp(x) \ee
 is also a local minimum of the convex composite problem 
\be \label{eq:soc:prob-misc6} \min_x~f(x) + \vp_d(F(x)) + \bar c, \ee 
for some constant $\bar c \in \R$, and vice versa. However, this analogy does not need to be true for the different notions of stationarity, i.e., a stationary point of the initial problem \eqref{eq:soc:prob-misc5} is not necessarily a stationary point of the composite problem \eqref{eq:soc:prob-misc6} in the sense of Definition \ref{definition:soc:stationarity}. Our earlier discussion in Remark \ref{remark:soc:stat-back} already showed that, in general, we can only expect the following implication
%
\[ \lagset(\bar x) \neq \emptyset \quad \implies \quad \FopL(\bar x) = 0, \]
%
where $\lagset(\bar x) = \{\lambda \in \partial \vp_d(F(\bar x)): \nabla f(\bar x) + DF(\bar x)^\top \lambda = 0 \}$ is the set of corresponding Lagrange multipliers of \eqref{eq:soc:prob-misc6} and $\Lambda \in \Spp$ is an arbitrary parameter matrix. Now, if the function $\vp$ is $C^\ell$-decomposable at some point $\bar x \in \dom~\vp$ with decomposition pair $(\vp_d,F)$, then Robinson's constraint qualification guarantees that these two different stationarity concepts are actually equivalent, i.e., we have
%
\[ \lagset(\bar x) \neq \emptyset \quad \iff \quad \FopL(\bar x) = 0. \]
%
Moreover, due to the stability property of Robinson's constraint qualification (see subsection \ref{sec:chap02:rob-cq}), the latter equivalence is also satisfied for any other stationary point that lies in a certain neighborhood of $\bar x$. Consequently, $\bar x$ is an isolated stationary point of our initial problem if and only if $\bar x$ is an isolated stationary point of the composite problem \eqref{eq:soc:prob-misc6}. Therefore, in the context of decomposable functions, there is no difference between these two stationarity concepts. Thus, the overall idea of decomposability and decomposable optimization problems can be summarized as follows. \vspace{1ex}

Let us suppose that the function $\vp$ is $C^\ell$-decomposable at a local minimum or a stationary point  $\bar x \in \dom~\vp$ of \eqref{eq:soc:prob-misc5}. Then, the second order analysis of $\bar x$ and of the initial problem \eqref{eq:soc:prob-misc5} can be completely transferred to the composite problem \eqref{eq:soc:prob-misc6}. Since the latter problem is a general convex composite problem of the form \eqref{eq:soc:prob1}, our abstract second order framework and theory of the sections \ref{sec:chap04:iso-stat} and \ref{section:soc:no gap} can be applied. Furthermore, due to the demonstrated, local equivalence of the problems \eqref{eq:soc:prob-misc5} and \eqref{eq:soc:prob-misc6}, any optimality and stationarity result that is obtained for the composite setting, can be passed to the original problem \eqref{eq:soc:prob-misc5}.  \end{remark}

In the following, we want to briefly assess the class of decomposable functions with respect to its generality and compare it to the so-called class of amenable functions, which was introduced by Poliquin and Rockafellar in \cite{PolRoc92,PolRoc93}.  

\begin{definition}[{cf. \cite[Definition 1.1 and 1.2]{PolRoc92}}] A function $\vp : \Rn \to \Rex$ is \rmn{amenable} at $\bar x \in \dom~\vp$ if there is an open neighborhood $U$ of $\bar x$ such that 
\[ \vp(x) = \vp_a(F(x)), \quad \forall~x \in U, \]
where $F : \Rn \to \Rm$ is a continuously differentiable function and $\vp_a : \Rm \to \Rex$ is a convex, proper, and lower semicontinuous mapping and the following basic constraint qualification is satisfied:
%
\begin{center} there is no $y \neq 0$ in $N_{\dom~\vp_a}(F(\bar x))$ with $DF(\bar x)^\top y = 0$. \end{center}
%
The function $\vp$ is called \rmn{fully amenable} if such a representation exists and, additionally, the function $F$ is twice continuously differentiable and $\vp_a$ is piecewise linear-quadratic. 
%Moreover,in this situation, $\varrho$ is called fully amenable if $\varrho_a$ can be taken to be piecewise linear-quadratic. 
\end{definition}

By \cite[Proposition 2.97 and Corollary 2.98]{BonSha00}, the basic constraint qualification is just an equivalent reformulation of Robinson's constraint qualification. Thus, any $C^1$-decomposable function is amenable. On the other hand, an amenable function is $C^1$-decomposable if and only if the function $\vp_a$ is additionally positively homogeneous and it holds $F(\bar x) = 0$. Moreover, it is also clear that a $C^2$-decomposable function does not need to be fully amenable and vice versa. Finally, in \cite{Sha03}, it was shown that a $C^2$-fully decomposable function is also \textit{partly smooth} in the sense of Lewis \cite{Lew02}. For a more detailed overview and discussion of these different decomposition concepts we refer to Hare \cite{Har04,Har06} and \cite{Sha03}. For instance, a comprehensive visualization of the connection between various classes of functions, including amenable, decomposable and partly smooth functions, can be found in \cite[Figure 1]{Har06}. \vspace{1ex} %\todo{More?} 

Let us also mention that in \cite{Har04,Har06} decomposability was defined and studied without explicitly assuming Robinson's constraint qualification. Here, we decided to add this extra regularity condition, since, from a practical point of view, it does not seem to be too restrictive and it notably simplifies the calculus and the overall analysis. In particular, it can be shown that many results for (fully) amenable functions, such as sum and chain rules for second order epiderivatives, do also hold for (fully) decomposable functions and that basic techniques and proofs can be expanded to the class of decomposable functions. 


==> experiment.tex <==
\section{Numerical Experiments}
\label{sec:ne}
In this section, we demonstrate the efficiency of the proposed algorithm on a sparse logistic regression and a nonconvex image compression problem. All experiments are performed using MATLAB R2020a on a laptop with Intel Core i7 9750h (6 cores and 12 threads) 3.5GHz and 16GB memory.

\subsection{Implementational Details}
\label{sec:parameter}

We first describe and discuss some general implementational details of \cref{algo2}. In the following, we will refer to \cref{algo2} as TRSSN. 

We start with a brief overview of the utilized parameters. Most of the parameters of our algorithm are fixed throughout the conducted numerical experiments. The trust region parameters used in \cref{algo3} are listed in \cref{table1}. When updating the trust region radius, we set $\Delta_{k+1}=\gamma_0\Delta_k$ if $\rho_k<\eta_1$ and $\Delta_{k+1}=\Delta_k$ if $\rho_k \in [\eta_1,\eta_2)$. In the case $\rho_k \geq \eta_2$, we choose $\Delta_{k+1}=\gamma_1\Delta_k$.

\begin{table}[t]
\centering
\begin{tabular}{ccccC{1.7cm}C{1.7cm}cccc} %l(left)居左显示 r(right)居右显示 c居中显示
\specialrule{1pt}{0pt}{0pt} \\[-1.5ex]
\multirow{2}*{Parameter} & \multicolumn{3}{c}{TR Radius} & \multicolumn{2}{c}{Acceptance Threshold} & \multicolumn{3}{c}{$\nu_k$ and ${\mathrm{pred}}_k$} \\ \cmidrule(lr){2-4} \cmidrule(lr){5-6} \cmidrule(lr){7-9}
& $\Delta_{\min}$ & $\gamma_0$ & $\gamma_1$  & $\eta_1$ & $\eta_2$ & $\alpha$ & $c_a$  & $p$ \\[0.5ex]
 \hline \\[-1.5ex]
  Value & $10^{-2}$ & $0.25$ & $2$ & $10^{-6}$ & $0.75$ & $0.2$ &$10^{-3}$ & $0.1$  \\[0.5ex]
\specialrule{1pt}{0pt}{0pt} \\[-1.5ex]
\end{tabular}
\caption{Parameters of the trust region method.}
\label{table1}
\end{table}

 

The parameter $\nu_k$ in the predicted reduction term $\mathrm{pred}_k$ is set as in \cref{eq:nuk-ak}. In particular, we select $a_k := c_a k^{\alpha/2}$ with $\alpha = 2p$ and $p \in (0,1)$. The specific choice of the parameters $c_a$, $\alpha$, and $p$ is given in \cref{table1}. The parameter $\nu_k$ then is chosen as:
%
\[   \nu_k=\min\{\nu,10^{-3}(n_{\mathcal S}(k))^{0.4}\|\prox{z_k+s_k}-x_k\|_{\Lambda}^{0.2}\}  \quad \text{and} \quad \Lambda=\lambda I, \; \lambda > 0. \]
%
Furthermore, $\tau$ and $\nu$ are set to satisfy the requirements in \ref{B1}. In our numerical experiments, we choose:
%
\[   \tau =\frac{2\lambda^2}{L^2+2\lambda^2} \cdot c_{\tau},\quad \nu= \frac12\min\left\{\tau, c_{\nu}\left[1-\frac\tau2\left(\frac{L^2}{2\lambda^2}+1\right)\right]\right\},                   \]
%
where $c_{\tau}=c_{\nu}=0.05$. The tolerances $\{\epsilon_k\}$ in the CG-method are chosen adaptively as $\epsilon_k=\min\{ \|\Fnor{z_k}\|^{2.5},0.01\}$. The maximal number of CG-iterations is limited to 10. 

Since we need to compare our normal map-based algorithm with other approaches, we first generate a comparable pair of initial points $x_0$ and $z_0$. Specifically, for given $x_0 \in \Rn$, we compute a corresponding initial point $z_0$ via: 
%
\[  z_0 = \argmin\limits_{\prox{z}=x_0}\|\Fnor{z}\|. \]
%
Fortunately, in our numerical experiments, this $z_0$ can always be computed explicitly.

The evaluation of the merit function $\mer$ requires an additional evaluation of the gradient $\nabla f$, which can cause higher computational costs. To avoid this computation, we first check the condition 
%
\be \label{eq:num-pmer} \psi(\prox{z_k+s_k})\geq \mer(z_k) \ee
%
and, in such case, we set $\rho_k=-1$. Notice that \cref{eq:num-pmer} implies $\mer(z_k+s_k)\geq \psi(\prox{z_k+s_k}) \geq \mer(z_k)$, i.e., we have $\rho_k\leq 0$ and this step would be rejected. Hence, we do not need to compute $\Fnor{z_k+s_k}$ in this case. Since we mainly consider large-scale problems, we will utilize a limited memory version of the quasi-Newton method. Based on the classical work \cite{byrd1994representations}, we implement the following compact form of the (L-)BFGS scheme
%
\[  B_{k}=\gamma_k I-\begin{bmatrix} S_k & Y_k  \end{bmatrix}  \begin{bmatrix} \frac{1}{\gamma_k}S_k^\top S_k  & \frac{1}{\gamma_k}\cL_k \\  \frac{1}{\gamma_k}\cL_k^\top  & -D_k  \end{bmatrix}^{-1} \begin{bmatrix} S_k^\top  \\ Y_k^\top   \end{bmatrix} \]
where
%
\[ S_k=[d_{k-m},...,d_{k-1}],\quad Y_k=[y_{k-m},...,y_{k-1}], \]
%
 $\cL_k$ is the strictly lower part of $S_k^\top Y_k$, $D_k$ is the diagonal part of $S_k^\top Y_k$, and $m \in \N$ is a memory parameter. We choose $\gamma_k$ as $\gamma_k= {y_k^\top y_k}/{(s_k^\top y_k)}$. 
If an algorithm utilizes a quasi-Newton technique, then we apply L-BFGS approximations with memory $m=10$.
 

\subsection{Sparse Logistic Regression}
\label{sec:logistic}
In our first numerical experiment, we consider a sparse logistic regression problem of the form:
%
\be\label{eq:logreg-prob} \min_{x}~\psi(x)=f(x)+\varphi(x),\quad f(x):=\frac{1}{N}\sum_{i=1}^{N}f_i(x),\quad\varphi(x):=\mu\|x\|_1, \ee
%
where $f_i(x):=\log(1+\exp(-b_i\cdot\langle a_i,x \rangle))$ denotes the logistic loss function and the data pairs $(a_i,b_i)\in\mathbb{R}^n\times\{-1,1\}$ are given for all $i\in[N]$.  The Lipschitz constant of $\nabla f$ can be computed explicitly via $L={\|A\|_2^2}/(4N)$, where $A=(a_1,...,a_N)^\top\in\mathbb{R}^{N\times n}$. For this example, the proximal operator is  the well-known shrinkage operator\begin{align}
\label{eq:l1prox}
  \mathrm{prox}^\Lambda_{\mu\|\cdot\|_1}(z) = \mathrm{prox}^{\lambda I}_{\mu\|\cdot\|_1}(z) =\max\left\{0,|z|-\frac{\mu}{\lambda}\right\}\odot \mathrm{sgn}(z),
\end{align}
%
where all the operations are understood componentwisely. Due to the separability of the $\ell_1$-norm, the generalized derivatives of the proximity operator $\mathrm{prox}^\Lambda_{\mu\|\cdot\|_1}$ at $z \in \Rn$ can be represented as diagonal matrices with
\begin{align}
\label{eq:generalizedjac}
D(z) = \mathrm{diag}(d(z)) \quad \text{and} \quad d_{i}(z) = 
\begin{cases}
0  &\text{if~~}|z_i|\leq \frac{\mu}{\lambda}, \\
1   & \text{otherwise}, 
\end{cases}
\end{align}
%
see, e.g., \cite{milzarek2014semismooth,milzarek2016numerical}. We set $\lambda=\min\{\frac{L}{2},0.4\}$, $\Lambda=\lambda I$, and $x^0 = 0$ in all of our experiments. We compare TRSSN with the following methods: 
\begin{itemize}
\item \textbf{PNOPT}~\cite{lee2014proximal}. \text{PNOPT} is a proximal Newton method which uses a quasi-Newton approximation of $\nabla^2f$ as parameter matrix $\Lambda$ in the proximal step. We use the source code released by the authors\footnote{\url{https://web.stanford.edu/group/SOL/software/pnopt/}}. All the parameters are set to be the default values as specified in the source code.
\item \textbf{ASSN}~\cite{xiao2018regularized}. \text{ASSN} is a semismooth Newton method for solving monotone equations. Following \cite[section 4.1]{xiao2018regularized} and  based on the source code provided by the authors, we implement ASSN with full Hessian information to solve the nonsmooth equation $F^{\lambda I}_{\mathrm{nat}}(x) = 0$. We have also tried an L-BFGS version of ASSN (called ASLB). However, its performance is not comparable with the base algorithm ASSN, which also agrees with an observation made in \cite[section 4.2]{xiao2018regularized}. Thus, we only report the numerical performance of ASSN here. Moreover, as noted in \cite{xiao2018regularized}, the parameter $\lambda$ should be no less than $L$ to ensure monotonicity of the natural residual $F^{\lambda I}_{\mathrm{nat}}$. So we choose $\lambda = L$ in the \text{ASSN} code.  
\item \textbf{FISTA}~\cite{beck2009fast}. \text{FISTA} is a first-order method with Nesterov-type acceleration. In our implementation, we use the known Lipschitz constant as step size.  
\item  \textbf{DAL}~\cite{tomioka2011super}. \text{DAL} is a dual augmented Lagrangian algorithm. We use the code released by the authors\footnote{\url{https://github.com/ryotat/dal}}. All parameters are set to default values.
\item \textbf{ForBES}~\cite{SteThePat17}. \text{ForBES} applies the semismooth Newton method to the natural residual $F^{\lambda I}_{\mathrm{nat}}$ using a forward-backward envelope as the merit function. We use the code provided by the authors\footnote{\url{https://github.com/kul-forbes/ForBES}}. We choose the Lipschitz constant $L$ as initial value for $\lambda$ and the released MATLAB function then corrects $\lambda$ to $\lambda={L}/{0.95}$. All other parameters are set to be default values.
\end{itemize}

\begin{table}[t]
  \centering
   \begin{tabular}{ccccccccc}  
 \cmidrule[1pt](){1-4} \cmidrule[1pt](){6-9} %\toprule%\specialrule{1pt}{0pt}{0pt} \\[-1.5ex]
  Dataset & $N$ & $n$ & Reference & & Dataset & $N$ & $n$ & Reference \\[0.5ex]  % \texttt{gisette} &   & \texttt{rcv1} \\
  \cmidrule(){1-4} \cmidrule(){6-9} \\[-1.5ex]
   \texttt{CINA} & 16\,033 & 132 & \cite{CINA} & & \texttt{gisette} & 6\,000 & 5\,000 & \cite{gisette} \\[0.5ex]
   \texttt{covtype} & 581\,012 & 54 & \cite{covtype} & & \texttt{rcv1} & 20\,242 & 47\,236 & \cite{RCV1} \\[0.5ex]
 \cmidrule[1pt](){1-4} \cmidrule[1pt](){6-9} \\[-1.5ex]
  \end{tabular}
  \caption{Information of the different datasets.}
  \label{table2}
  \end{table}

We have tested TRSSN and the mentioned algorithms on four different datasets (\texttt{CINA}, \texttt{covtype}, \texttt{gisette}, and \texttt{rcv1}). More information about these datasets can be found in \cref{table2}. The results of our comparison are shown in \cref{fig2} and \cref{fig2b}. Specifically, in \cref{fig2} and \cref{fig2b}, we plot the relative error $\texttt{rel$\_$err} = (\psi(x)-\psi^*) /\max\{1,\psi^*\}$ with respect to the number of iterations and cpu-time. Here, $\psi^*$ is the lowest objective function value encountered by all the algorithms during the experiment. 

In terms of iterations, the methods ForBES, PNOPT, and TRSSN achieve the best results and outperform the accelerated first-order approach FISTA and the augmented Lagrangian method DAL on all datasets. PNOPT seems to perform especially well in its early stage and it can quickly recover solutions with medium accuracy. However, PNOPT stagnates and converges slower when a higher precision ($\geq 10^{-8}$) is required. We note that \text{DAL} performs inner iterations that only update a dual variable. Hence, the function values $\psi(x)$ can only be updated in outer iterations which explains the different convergence behavior of DAL reported in \cref{fig2} and \cref{fig2b}. On the dataset \texttt{covtpye} and \texttt{rcv1}, ASSN performs well and transition to fast local convergence can be observed (we believe that a more problem dependent and tuned choice of the involved parameters can also lead to earlier fast local convergence on the other datasets). Concerning cpu-time, TRSSN outperforms almost all of the other tested algorithms. We notice that ForBES and PNOPT utilize line search to damp the second-order step and to ensure convergence and ASSN utilizes alternative projection steps if the semismooth Newton step does not satisfy a certain acceptance criterion. In contrast, our trust region-type framework (paired with the inexact Steihaug CG-method) requires less computational steps and gradient and function values can be fully reused in case a trial step is unsuccessful. 
 

In \cref{fig1}, we discuss the performance of TRSSN on the datasets \texttt{CINA} and \texttt{rcv1} for different choices of the L-BFGS memory parameter $m$. We have also included additional runs of TRSSN using full Hessian information. The results in \cref{fig1} demonstrate that full Hessian information can be beneficial in certain situations to further reduce the number of iterations. However, the computational costs per iteration can then also be higher as shown in \cref{fig1} (b). It turns out that the numerical performance of TRSSN with L-BFGS updates is not very sensitive to the choice of $m$.
  
\begin{figure}[t]
\centering
\begin{tikzpicture}[scale=1]
\draw[black] (0,0)--(15.6,0)--(15.6,0.5)--(0,0.5)--(0,0);
\fill[redp] (0.3,0.2)--(0.7,0.2)--(0.7,0.3)--(0.3,0.3)--cycle;
\node[right] at (0.75,0.25) {PNOPT};
\fill[orangep] (2.9,0.2)--(3.3,0.2)--(3.3,0.3)--(2.9,0.3)--cycle;
\node[right] at (3.35,0.25) {ASSN};
\fill[yellowp] (5.5,0.2)--(5.9,0.2)--(5.9,0.3)--(5.5,0.3)--cycle;
\node[right] at (5.95,0.25) {FISTA};
\fill[greenp] (8.1,0.2)--(8.5,0.2)--(8.5,0.3)--(8.1,0.3)--cycle;
\node[right] at (8.55,0.25) {ForBES};
\fill[bluep] (10.7,0.2)--(11.1,0.2)--(11.1,0.3)--(10.7,0.3)--cycle;
\node[right] at (11.15,0.25) {DAL};
\fill[purplep] (13.3,0.2)--(13.7,0.2)--(13.7,0.3)--(13.3,0.3)--cycle;
\node[right] at (13.75,0.25) {TRSSN};
\end{tikzpicture}

\subfigure[\texttt{CINA}.]{
\includegraphics[width=7.5cm]{figure/CINA_iteration.pdf}
}
\quad
\subfigure[\texttt{covtype}.]{
\includegraphics[width=7.5cm]{figure/covtype_iteration.pdf}
}
\quad
\subfigure[\texttt{gisette}.]{
\includegraphics[width=7.5cm]{figure/gisette_iteration.pdf} 
                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                   }
\quad
\subfigure[\texttt{rcv1}.]{
\includegraphics[width=7.5cm]{figure/rcv1_iteration.pdf} 
}
\caption{Change of the relative error $\texttt{rel$\_$err}$ with respect to the number of iterations for solving the $\ell_1$-logistic
regression problem \cref{eq:logreg-prob}.}
\label{fig2}
\end{figure} 

\begin{figure}[htbp]
\centering
\begin{tikzpicture}[scale=1]
\draw[black] (0,0)--(15.6,0)--(15.6,0.5)--(0,0.5)--(0,0);
\fill[redp] (0.3,0.2)--(0.7,0.2)--(0.7,0.3)--(0.3,0.3)--cycle;
\node[right] at (0.75,0.25) {PNOPT};
\fill[orangep] (2.9,0.2)--(3.3,0.2)--(3.3,0.3)--(2.9,0.3)--cycle;
\node[right] at (3.35,0.25) {ASSN};
\fill[yellowp] (5.5,0.2)--(5.9,0.2)--(5.9,0.3)--(5.5,0.3)--cycle;
\node[right] at (5.95,0.25) {FISTA};
\fill[greenp] (8.1,0.2)--(8.5,0.2)--(8.5,0.3)--(8.1,0.3)--cycle;
\node[right] at (8.55,0.25) {ForBES};
\fill[bluep] (10.7,0.2)--(11.1,0.2)--(11.1,0.3)--(10.7,0.3)--cycle;
\node[right] at (11.15,0.25) {DAL};
\fill[purplep] (13.3,0.2)--(13.7,0.2)--(13.7,0.3)--(13.3,0.3)--cycle;
\node[right] at (13.75,0.25) {TRSSN};
\end{tikzpicture}

\subfigure[\texttt{CINA}.]{
\includegraphics[width=7.5cm]{figure/CINA_times.pdf}
}
\quad
\subfigure[\texttt{covtype}.]{
\includegraphics[width=7.5cm]{figure/covtype_times.pdf} 
}
\quad
\subfigure[\texttt{gisette}.]{
\includegraphics[width=7.5cm]{figure/gisette_times.pdf}
}
\quad
\subfigure[\texttt{rcv1}.]{
\includegraphics[width=7.5cm]{figure/rcv1_times.pdf}
}
\caption{Change of the relative error $\texttt{rel$\_$err}$ with respect to the cpu-time for solving the $\ell_1$-logistic
regression problem \cref{eq:logreg-prob}.}
\label{fig2b}
\end{figure} 


\begin{figure}[htbp]
\centering
\begin{tikzpicture}[scale=1]
\draw[black] (0,0.5)--(15.6,0.5)--(15.6,-0.5)--(0,-0.5)--(0,0.5);
\fill[redp] (0.3,0.2)--(0.7,0.2)--(0.7,0.3)--(0.3,0.3)--cycle;
\node[right] at (0.75,0.25) {TRSSN $m=5$};
\fill[orangep] (4.2,0.2)--(4.6,0.2)--(4.6,0.3)--(4.2,0.3)--cycle;
\node[right] at (4.65,0.25) {TRSSN $m=10$};
\fill[yellowp] (8.1,0.2)--(8.5,0.2)--(8.5,0.3)--(8.1,0.3)--cycle;
\node[right] at (8.55,0.25) {TRSSN $m=20$};
\fill[greenp] (11.7,0.2)--(12.1,0.2)--(12.1,0.3)--(11.7,0.3)--cycle;
\node[right] at (12.15,0.25) {TRSSN $m=30$};
\fill[bluep] (0.3,-0.2)--(0.7,-0.2)--(0.7,-0.3)--(0.3,-0.3)--cycle;
\node[right] at (0.75,-0.25) {TRSSN $m=40$};
\fill[purplep] (4.2,-0.2)--(4.6,-0.2)--(4.6,-0.3)--(4.2,-0.3)--cycle;
\node[right] at (4.65,-0.25) {TRSSN $m=50$};
\fill[brownp] (8.1,-0.2)--(8.5,-0.2)--(8.5,-0.3)--(8.1,-0.3)--cycle;
\node[right] at (8.55,-0.25) {TRSSN Full Hess.};
\fill[ivory] (11.7,-0.2)--(12.1,-0.2)--(12.1,-0.3)--(11.7,-0.3)--cycle;
\node[right] at (12.15,-0.25) {ASSN};
\end{tikzpicture}

\subfigure[\texttt{CINA} -- iterations.]{
\includegraphics[width=7.5cm]{figure/CINA_different_m_iteration.pdf}
}
\quad
\subfigure[\texttt{CINA} -- cpu-time.]{
\includegraphics[width=7.5cm]{figure/CINA_different_m_times.pdf}
}
\quad
\subfigure[\texttt{rcv1} -- iterations.]{
\includegraphics[width=7.5cm]{figure/rcv1_different_m_iteration.pdf}
}
\quad
\subfigure[\texttt{rcv1} -- cpu-time.]{
\includegraphics[width=7.5cm]{figure/rcv1_different_m_times.pdf}
}
 
\caption{Results for the logistic regression problem. Comparison of TRSSN on \texttt{CINA} and \texttt{rcv1} for different choices of the L-BFGS memory parameter $m$.}
\label{fig1}
\end{figure} 



\subsection{Linear Diffusion Based Image Compression}
Next, we test TRSSN on a linear diffusion based image compression problem. The compression model we consider has been studied in  \cite{galic2008image,schmaltz2009beating}.  
The model utilizes a homogeneous diffusion based interpolation to find the optimal data. The associated optimization formulation is given by 
%
\begin{align}
\min\limits_{x,c}~\frac{1}{2}\|x-u\|^2+\lambda\|c\|_1 \quad
\mathrm{s.t.}\quad \diag(c)(x-u)-(I-\diag(c))\mathcal L u=0, \label{eq9-1}
\end{align}
where $u\in\mathbb{R}^N$ denotes the (stacked) ground truth image, $x\in\mathbb{R}^N$ is the reconstructed image, $c\in\mathbb{R}^N$ denotes the inpainting or compression mask, and $\mathcal L \in \R^{N \times N}$ is the discretized Laplacian. If $c\neq 0$ and $c\in[0,1]^n$, then the matrix $A(c):=\diag(c)+(\diag(c)-I)\mathcal L$ can be shown to be invertible \cite{MaiBruWeiFor11}. Setting $x=A(c)^{-1}\diag(c)u$, problem $\cref{eq9-1}$ can then be rewritten as:
\begin{align*}
\min_c~\frac{1}{2}\|A(c)^{-1}\diag(c)u-u\|^2+\mu\|c\|_1 \quad \mathrm{s.t.} \quad c\in [0,1]^n.
\end{align*}
Thus, problem \cref{eq9-1} reduces to the standard form in \cref{eq1-1} with $f(c)=\frac{1}{2}\|A(c)^{-1}\diag(c)u-u\|^2$ and $\varphi(c)=\lambda\|c\|_1+\iota_{[0,1]^n}(c)$. By \cite[Lemma 5.2]{OchCheBroPoc14}, the gradient of $f$ can be calculated as follows
\begin{align}
\label{eq9-2}
 \nabla f(c)=\diag(-\mathcal L x+u-x)[A(c)^{\top}]^{-1}(x-u)\quad \text{where} \quad x=A(c)^{-1}\diag(c)u. 
\end{align}

Since the Lipschitz constant of $\nabla f$ can not be computed exactly, we use an adaptive strategy for choosing $L$. First, we select an initial estimate $L_0$. In each trial step, we then calculate $c_{k+1}=\prox{z_k+s_k}$ and choose $$L_k=\max\left\{2\cdot\frac{f(c_{k+1})-f(c_k)-\langle \nabla f(c_k),c_{k+1}-c_k\rangle}{\|c_{k+1}-c_k\|^2},2L_{k-1}\right\}.$$
We reset $\Lambda=L_k I$ and adjust $\nu$ and $\tau$ as specified in \cref{sec:parameter}. In all of our examples, we choose $L_0 = 0.1$.

The proximity operator is slightly different to the one in \cref{sec:logistic}. According to~\cite[Theorem 1]{yu2013decomposing}, we have
%
\[  \prox{z}=\mathcal P_{[0,1]^n}\circ\mathrm{prox}^{\lambda I}_{\mu \|\cdot\|_1}(z)=\min\{0,\max\{1,\mathrm{prox}^{\lambda I}_{\mu \|\cdot\|_1}(z)\}\},       \]
%
where the explicit form of $\mathrm{prox}^{\lambda I}_{\mu \|\cdot\|_1}(z)$ can be found in \cref{eq:l1prox} and all operations are understood componentwisely. The corresponding generalized derivative of this proximity operator can be constructed similarly to \cref{eq:generalizedjac}. Here, we choose
%
\begin{align*}
D(z) = \mathrm{diag}(d(z)) \quad \text{and} \quad d_{i}(z)= 
\begin{cases}
0 &  \text{if } z_i\leq \frac{\mu}{\lambda} \; \text{ or } \; z_i\geq \frac{\mu}{\lambda}+1 , \\
1 & \text{otherwise},
\end{cases}
\end{align*}

see, e.g., \cite[Example 4.2.17]{milzarek2016numerical} for comparison. Because this problem is nonconvex, most of the algorithms tested in \cref{sec:logistic} are no longer directly applicable. We compare our method with the following algorithms:
\begin{itemize}
\item \textbf{ForBES}~\cite{SteThePat17}. We use the same source code as in \cref{sec:logistic}. In the ForBES code, $f$ is assumed to be defined on the whole $\Rn$ which is not the case for \cref{eq9-1}. To apply ForBES to \cref{eq9-1}, we have tested two strategies. The first variant, referred to as ForBES-S1, sets $f$ to $+\infty$ outside of the effective domain of $\varphi$. In our second strategy, ForBES-S2, $\nabla f$ is computed using \cref{eq9-2} regardless of the constraint $c\in[0,1]^n$. Unfortunately, both strategies cost too much time to converge to a reasonable solution. For ForBES-S1, the line search strategy typically reaches the maximum number of iterations. Specifically, if some of the components of $x_k$ are exactly $0$ (or $1$) and the corresponding components of the descent direction $d_k$ are negative (positive), then the line search step in \cite{SteThePat17} would stagnate and fail at this point. This is very likely to happen when the dimension of the problem is large. For ForBES-S2, we observe that the evaluation of the forward-backward envelope is very time-consuming since it involves the computation of the full gradient. In addition, backtracking requires a relatively high number of steps to converge since $f$ and the forward-backward envelope change sharply when $x_k$ is close to the boundary of $[0,1]^n$. In our tests, ForBES-S2 needs around 24 hours to run 2500 iterations for a $512\times 512$ input image. Due to these limitations, we will not report the performance of ForBES here.    
\item \textbf{iPiano}~\cite{OchCheBroPoc14}. \text{iPiano} is a first-order method applying momentum acceleration to forward-backward splitting. We implement this algorithm with backtracking following the recommendations in \cite{OchCheBroPoc14}. As in  \cite{OchCheBroPoc14}, we set $\alpha={1.99(1-\beta)}/{L}$, $\eta=2$, and $\beta=0.8$. The initial Lipschitz constant $L_0$ is set to be $0.1$. As suggested in \cite{OchCheBroPoc14}, we increase the Lipschitz constant $L$ adaptively by $5\%$ after every five steps. 
\item \textbf{SpaRSA}~\cite{WriNowFig09}. \text{SpaRSA} is a proximal gradient method with Barzilai-Borwein step sizes.  We implement this algorithm based on the source code provided by the authors\footnote{\url{https://www.lx.it.pt/~mtf/SpaRSA/}}. In SpaRSA, we set 
%
\[ \alpha_k = \frac{(r_k)^\top r_k}{(r_k)^\top s_k}, \quad r_k = \nabla f(c_k)-\nabla f(c_{k-1}), \quad s_k = c_k - c_{k-1}, \]  
%
as initial step size as suggested by the authors, see \cite[section II.E]{WriNowFig09}. Moreover, as in \cite{WriNowFig09}, the lower and upper bounds on $\alpha_k$ are given by $\alpha_{\min}=10^{-30}$ and $\alpha_{\max}=10^{30}$. Following a strategy proposed in \cite{WenYinGolZha10}, we utilize the nonmonotone line search procedure developed in \cite{ZhaHag04} to ensure global convergence of the approach and stability of the Barzilai-Borwein step sizes. 
\end{itemize}
Our results are summarized and shown in \cref{fig3}--\cref{fig4}. We compare the performance of the algorithms on the four different images \texttt{books}, \texttt{coffee}, \texttt{mountain}, and \texttt{stones}\footnote{Image credentials: \texttt{books} by Suzy Hazelwood; \texttt{coffee} by Atichart Wongubon; \texttt{mountain} by Denis Linine; \texttt{stones} by Travel Photographer; all images can be found on StockSnap.}. All images have been rescaled to size $512\times 512$ and we use $\mu = 0.01$ for \texttt{books}, $\mu = 0.003$ for \texttt{coffee} and \texttt{stones}, and $\mu = 0.02$ for \texttt{mountain}. In all tested examples, the performance of SpaRSA and iPiano is quite similar, while iPiano is generally more stable. Moreover, both SpaRSA and iPiano have large fluctuations throughout the iterative process (and on all tested images). As demonstrated in \cref{fig3} and \cref{fig3-2}, TRSSN significantly outperforms the other first-order approaches both in terms of the number of iterations and cpu-time. In addition, the overall performance of TRSSN appears to be more stable. 

\begin{figure}[t]
\centering
\begin{tikzpicture}[scale=1]
\draw[black] (0,0)--(15.6,0)--(15.6,0.5)--(0,0.5)--(0,0);
\fill[redp] (0.3,0.2)--(0.7,0.2)--(0.7,0.3)--(0.3,0.3)--cycle;
\node[right] at (0.75,0.25) {iPiano};
\fill[yellowp] (5.5,0.2)--(5.9,0.2)--(5.9,0.3)--(5.5,0.3)--cycle;
\node[right] at (5.95,0.25) {Sparsa};
\fill[bluep] (10.7,0.2)--(11.1,0.2)--(11.1,0.3)--(10.7,0.3)--cycle;
\node[right] at (11.15,0.25) {TRSSN};
\end{tikzpicture}

\subfigure[\texttt{books} -- iterations.]{
\includegraphics[width=7.5cm]{figure/512_512_books_iteration.pdf}
}
\quad
 \subfigure[\texttt{coffee} -- iterations.]{
\includegraphics[width=7.5cm]{figure/512_512_coffee_iteration.pdf}
}
\quad
\subfigure[\texttt{mountain} -- iterations.]{
\includegraphics[width=7.5cm]{figure/512_512_mountain_iteration.pdf}
}
\quad
\subfigure[\texttt{stones} -- iterations.]{
\includegraphics[width=7.5cm]{figure/512_512_stones_iteration.pdf}
}
\caption{Numerical comparison of iPiano, SpaRSA, and TRSSN on a diffusion based image compression problem. Plot of the norm of the natural residual with respect to required iterations for different images.}
\label{fig3}
\end{figure} 

\begin{figure}[htbp]
\centering
\begin{tikzpicture}[scale=1]
\draw[black] (0,0)--(15.6,0)--(15.6,0.5)--(0,0.5)--(0,0);
\fill[redp] (0.3,0.2)--(0.7,0.2)--(0.7,0.3)--(0.3,0.3)--cycle;
\node[right] at (0.75,0.25) {iPiano};
\fill[yellowp] (5.5,0.2)--(5.9,0.2)--(5.9,0.3)--(5.5,0.3)--cycle;
\node[right] at (5.95,0.25) {Sparsa};
\fill[bluep] (10.7,0.2)--(11.1,0.2)--(11.1,0.3)--(10.7,0.3)--cycle;
\node[right] at (11.15,0.25) {TRSSN};
\end{tikzpicture}

\subfigure[\texttt{books} -- cpu-time.]{
\includegraphics[width=7.5cm]{figure/512_512_books_times.pdf}
}
\quad
\subfigure[\texttt{coffee} -- cpu-time.]{
\includegraphics[width=7.5cm]{figure/512_512_coffee_times.pdf}
}
\quad
\subfigure[\texttt{mountain} -- cpu-time.]{
\includegraphics[width=7.5cm]{figure/512_512_mountain_times.pdf}
}
\quad
\subfigure[\texttt{stones} -- cpu-time.]{
\includegraphics[width=7.5cm]{figure/512_512_stones_times.pdf}
}
\caption{Numerical comparison of iPiano, SpaRSA, and TRSSN on a diffusion based image compression problem. Plot of the norm of the natural residual with respect to required cpu-time for different images.}
\label{fig3-2}
\end{figure} 

\begin{figure}[htbp]
\centering
\subfigure[\texttt{books} -- original figure.]{
\includegraphics[width=4.5cm]{figure/books512_t1.png}
}
\subfigure[\texttt{books} -- mask (${ds} = 8.43\%$).]{
\includegraphics[width=4.5cm]{figure/mask_trssn_books_512_t1.png}
}
\subfigure[\texttt{books} -- reconstruction.]{
\includegraphics[width=4.5cm]{figure/rec_trssn_books_512_t1.png}
}
\subfigure[\texttt{coffee} -- original figure.]{
\includegraphics[width=4.5cm]{figure/coffee512_t1.png}
}
\subfigure[\texttt{coffee} -- mask (${ds} = 4.45\%$).]{
\includegraphics[width=4.5cm]{figure/mask_trssn_coffee_512_t1.png}
}
\subfigure[\texttt{coffee} -- reconstruction.]{
\includegraphics[width=4.5cm]{figure/rec_trssn_coffee_512_t1.png}
}
\subfigure[\texttt{mountain} -- original figure.]{
\includegraphics[width=4.5cm]{figure/mountain512_t1.png}
}
\subfigure[\texttt{mountain} -- mask (${ds} = 3.99\%$).]{
\includegraphics[width=4.5cm]{figure/mask_trssn_mountain_512_t1.png}
}
\subfigure[\texttt{mountain} -- reconstruction.]{
\includegraphics[width=4.5cm]{figure/rec_trssn_mountain_512_t1.png}
}
\subfigure[\texttt{stones} -- original figure.]{
\includegraphics[width=4.5cm]{figure/stones512_t1.png}
}
\subfigure[\texttt{stones} -- mask (${ds} = 4.37\%$).]{
\includegraphics[width=4.5cm]{figure/mask_trssn_stones_512_t1.png}
}
\subfigure[\texttt{stones} -- reconstruction.]{
\includegraphics[width=4.5cm]{figure/rec_trssn_stones_512_t1.png}
}
\caption{Illustration of the different ground truth images, the inpainting or compression masks, and the corresponding reconstructions. The density ($ds$) of the masks $c$ is calculated via ${ds} := 100\% \cdot [ |\{i: c_i > 0\}| / (512 \times 512)]$.}
\label{fig4}
\end{figure} 

==> experiment_old.tex <==
\section{Numerical Experiments}
\label{sec:ne}
We demonstrate the efficiency of the proposed algorithm by conducting several numerical experiments. All the experiments are performed using MATLAB R2020a on a laptop with Intel Core i7 9750h (6 cores and 12 threads) 3.5GHz and 16GB memory.

\revised{We mainly consider large-scale problems in this paper}, which motivates the use of limited memory version of quasi-Newton method. The BFGS update used in our paper \revised{is based on the classical work} \cite{byrd1994representations}. It mainly relies on the compact form of BFGS update:
$$  B_{k}=\gamma_k I-\begin{bmatrix} S_k & Y_k  \end{bmatrix}  \begin{bmatrix} \frac{1}{\gamma_k}S_k^TS_k  & \frac{1}{\gamma_k}L_k \\  \frac{1}{\gamma_k}L_k^T & -D_k  \end{bmatrix}^{-1} \begin{bmatrix} S_k^T \\ Y_k^T  \end{bmatrix}                         $$
where
$$S_k=[d_{k-m},...d_{k-1}],\quad Y_k=[y_{k-m},...y_{k-1}],$$
 $L_k$ is the strictly lower part of $S_k^TY_k$, and $D_k$ is the diagonal part of $S_k^TY_k$. For the choice of $\gamma_k$, we follow the standard choice that $\gamma_k=\frac{y_k^Ty_k}{s_k^Ty_k}$. Moreover, since we utilize limited memory strategy, the norm $\|B_k\|$ is bounded as long as $\gamma_k$ remains bounded. So in the code we do not add the safe-guard operation in line 4 of Algorithm~\ref{algo-4}. Moreover, for all the algorithms including our algorithm mentioned in this section, if quasi-Newton technique is used, then we apply LBFGS approximations with memory $m=10$.
 
\subsection{Parameter Setting}
\label{sec:parameter}
Most of the parameters are fixed for all the numerical experiments. 

The trust-region parameters used in Algorithm~\ref{algo3} are listed in Table~\ref{table1}. For the update of $\Delta_k$, if $\rho_k<\eta_1$ then we set $\Delta_{k+1}=\gamma_0\Delta_k$, else if $\eta_1<=\rho_k<\eta_2$ we set $\Delta_{k+1}=\Delta_k$, otherwise $\Delta_{k+1}=\gamma_1\Delta_k$.

\begin{table}[h]
\centering
 \begin{tabular}{|c|c|c|c|c|c|c|c|c|c|} %l(left)居左显示 r(right)居右显示 c居中显示
\hline
Parameter & $\Delta_{\min}$ & $\gamma_0$ & $\gamma_1$  & $\eta_1$  & $\eta_2$ & $\alpha$ & $c_a$  & $p$   \\
 \hline
  Value & $10^{-2}$ & $0.25$ & $2$ & $10^{-6}$ & $0.75$ & $0.2$ &$10^{-3}$ & $0.1$  \\
  \hline
\end{tabular}
\caption{Parameters for the trust-region method.}
\label{table1}
\end{table}

For the parameter used in the merit function, we mainly need to decide the series $\{a_k\}$ in Remark~\ref{remark-nuk}. The choice of $\alpha, ~c_a,~ p$ are all listed in Table~\ref{table1}. In this case we have
\[   \nu_k=\min\{\nu,10^{-3}(n_{\mathcal S}(k))^{0.4}\|\prox{z_k+s_k}-x_k\|_{\Lambda}^{0.2}\}     .\]
Moreover, the choice of $\tau$ and $\nu$ is specified in (B.1). In the numerical experiment, we set:
\[   \tau = c_{\tau}\frac{2\lambda^2}{L^2+2\lambda^2},\nu= \frac12\min\left\{\tau, c_{\nu}\left[1-\tau(\frac{L^2}{2\lambda^2}+1)/2\right]\right\},                   \]
where $c_{\tau}=c_{\nu}=0.05$ and $\Lambda=\lambda I$. 

For the parameters used in  Algorithm~\ref{algo2}, the tolerance $\epsilon_k$ in the CG step is set as $\epsilon_k=\min\{ \|\Fnor{z_k}\|^{2.5},0.01\}$. The maximal number of CG iterations is set to be 10. 

Since we need to compare our algorithm with other algorithms, which typically do not have an initial value $z_0$ and only $x_0$ is specified. To achieve a fair comparison, we compute $z_0$ given $x_0$ by the following formula:
\[  z_0=\argmin\limits_{\prox{z}=x_0}\|\Fnor{z}\|         \]
Fortunately, in our numerical experiments, $z_0$ can be computed explicitly.
\subsection{Implementation Details}
The evaluation of merit function $\mer$ contains $\nabla f$ which might cause additional computational costs. To avoid this computation, we check if $\psi(\prox{z_k+s_k})\geq \mer(z_k)$ firstly, and if so, we set $\rho_k=-1$. Because if $\psi(\prox{z_k+s_k})\geq \mer(z_k)$ then $\mer(z_k+s_k)\geq \psi(\prox{z_k+s_k}) \geq \mer(z_k)$, so $\rho_k\leq 0$ and this step would be rejected, which means there is no necessity to compute $\Fnor{z_k+s_k}$ in this case.

 

\subsection{Sparse Logistic Regression}
\label{sec:logistic}
In our first numerical experiment, we consider a sparse logistic regression problem of the form:
$$\min_{x}\psi(x)=f(x)+\varphi(x),\quad f(x):=\frac{1}{N}\sum_{i=1}^{N}f_i(x),\quad\varphi(x):=\mu\|x\|_1$$
where $f_i(x):=\log(1+\exp(-b_i\cdot\langle a_i,x \rangle))$ denotes the logistic loss function and the pairs $(a_i,b_i)\in\mathbb{R}^n\times\{-1,1\}$ for all $i\in[N]$.  The Lipschitz constant of $\nabla f$ can be computed explicitly via $L=\frac{\|A\|_2^2}{4N}$. For this example, the proximal operator is  the well-known shrinkage operator\begin{align}
\label{eq:l1prox}
  \prox{z}=\max\left\{0,|z|-\frac{\mu}{\lambda}\right\}\cdot \mathrm{sgn}(z),
\end{align}

where all the operations are understood componentwise and $\Lambda=\lambda I$. The generalized Jacobian of $\oprox$ is chosen to be a diagonal matrix whose diagonal element is defined as in~\cite[Example 4.2.16]{milzarek2016numerical}
\begin{align}
\label{eq:generalizedjac}
D_{ii}(z)=\left\{
\begin{aligned}
&0  &\mathrm{if~~}|z_i|\leq \frac{\mu}{\lambda} \\
&1   & \mathrm{otherwise}
\end{aligned}
\right.
\end{align}
We set $\Lambda=\min\{\frac{L}{2},0.4\}I$ for all the examples. In our experiment, we compare our algorithm TRSSN with the following algorithms: 
\begin{itemize}
\item PNOPT~\cite{lee2014proximal}. PNOPT is a proximal Newton method which uses a quasi-Newton approximation of $\nabla^2f$ in the proximal step. We use the source code released by the authors\footnote{\url{https://web.stanford.edu/group/SOL/software/pnopt/}}. All the parameters are set to be the default value as specified in their source code.
\item ASSN~\cite{xiao2018regularized}. ASSN is a semismooth Newton method for solving monotone nonsmooth equations. We implement this algorithm with full Hessian based on the source code provided by the authors. We also tried LBFGS implementation, but its performance is not comparable to other algorithms, which also agrees with the observation in \cite{xiao2018regularized}. So we do not report the numerical performance of the LBFGS version of ASSN. Moreover, it's noted in \cite{xiao2018regularized} that $\lambda$ should be no less than $L$ to ensure the monotonicity of the natural residual, so we choose $\Lambda=LI$ in the ASSN code.  
\item FISTA~\cite{beck2009fast}. FISTA is a first-order method with Nesterov's acceleration. We implement this algorithm by ourselves because no other additional parameter needs to be specified. We use the known Lipschitz constant in the code.  
\item  DAL~\cite{tomioka2011super}. DAL is a dual augmented Lagrangian algorithm. We use the code released by the authors\footnote{\url{https://github.com/ryotat/dal}}. All the parameters are set to be the default value.
\item ForBES~\cite{stella2017forward}. ForBES applies the semismooth Newton method to the natural residual using a forward-backward envelope as the merit function. We use the code released by the authors\footnote{\url{https://github.com/kul-forbes/ForBES}}. For the choice of $\Lambda$ we set the Lipschitz constant in the matlab function to be $L$ and the code chooses $\Lambda=\frac{L}{0.95}I$. All the other parameters are set to be default value.
\end{itemize}
The result is shown in Fig.\ref{fig1}. We have tested these algorithms on  4 datasets (covtype, gisette, CINA, rcv1). Specifically, we plot the ratio between $\psi-\psi_0$ and $\psi-\psi^*$, where $\psi^*$ is the optimal function value and is defined as the lowest function value encountered in all the algorithms. We note that due to DAL only update dual variable in the inner iterations, so its function value would be of the same among these inner iterations. The time cost for each iteration of our algorithm is the lowest one because when a step is unsuccessful, then the gradient and function value can be reused in the next iteration, and we do not need to do line-search as ForBES, DAL, PNOPT. The iteration picture also counts unsuccessful steps.

We also have tested the effect of different memory number and the use of full Hessian on the numerical performance, as shown in Fig.~\ref{fig2}. The tested datasets are CINA and rcv1.
 
\begin{figure}[htbp]
\centering
\subfigure[Iteration for covtype.]{
\includegraphics[width=6cm]{figure/covtype_iteration.pdf}
}
\quad
\subfigure[Time for covtype.]{
\includegraphics[width=6cm]{figure/covtype_times.pdf}
}
\quad
\subfigure[Iteration for gisette.]{
\includegraphics[width=6cm]{figure/gisette_iteration.pdf}
}
\quad
\subfigure[Time for gisette.]{
\includegraphics[width=6cm]{figure/gisette_times.pdf}
}
\quad
\subfigure[Iteration for CINA.]{
\includegraphics[width=6cm]{figure/CINA_iteration.pdf}
}
\quad
\subfigure[Time for CINA.]{
\includegraphics[width=6cm]{figure/CINA_times.pdf}
}
\quad
\subfigure[Iteration for rcv1.]{
\includegraphics[width=6cm]{figure/rcv1_iteration.pdf}
}
\quad
\subfigure[Time for rcv1.]{
\includegraphics[width=6cm]{figure/rcv1_times.pdf}
}
\caption{Results for logistic regression problem. The value $\psi^*$ is the optimal function value which is chosen as the minimal value appeared in all the algorithms, and $\psi_0$ is the initial function value. }
\label{fig2}
\end{figure} 


\begin{figure}[htbp]
\centering
\subfigure[Iteration for CINA.]{
\includegraphics[width=6cm]{figure/CINA_different_m_iteration.pdf}
}
\quad
\subfigure[Time for CINA.]{
\includegraphics[width=6cm]{figure/CINA_different_m_times.pdf}
}
\quad
\subfigure[Iteration for rcv1.]{
\includegraphics[width=6cm]{figure/rcv1_different_m_iteration.pdf}
}
\quad
\subfigure[Time for rcv1.]{
\includegraphics[width=6cm]{figure/rcv1_different_m_times.pdf}
}
 
\caption{Results for logistic regression problem. The value $\psi^*$ is the optimal function value which is chosen as the minimal value appeared in all the algorithms, and $\psi_0$ is the initial function value. .}
\label{fig1}
\end{figure} 



\subsection{Linear diffusion based image compression}
In this example we test TRSSN on linear diffusion based image compression. Former works \cite{galic2008image,schmaltz2009beating} have studied the efficiency of this model in the compression of image, which can outperform the JPEG2000. We will compare our algorithm with ipiano proposed by \cite{ochs2014ipiano}. This problem is to find the optimal data for homogeneous diffusion based interpolation, which can be
formulated as the follows:
\begin{align}
\min\limits_{x,c}\quad\frac{1}{2}\|x-u\|^2+\lambda\|c\|_1,\quad
\mathrm{s.t.}\quad \diag(c)(x-u)-(I-\diag(c))Lu=0 \label{eq9-1}
\end{align}
where $u\in\mathbb{R}^N$ denotes the ground truth image, $x\in\mathbb{R}^N$ denotes the reconstructed image,
and $c\in\mathbb{R}^N$ denotes the inpainting mask. If $c\neq 0$ and $c\in[0,1]^n$, then matrix $A(c):=\diag(c)+(\diag(c)-I)L$ can be proved to be invertible and hence $x=A(c)^{-1}\diag(c)u$. Then problem $\eqref{eq9-1}$ can be rewritten as:
\begin{align*}
\min_c\frac{1}{2}\|A(c)^{-1}\diag(c)u-u\|^2+\mu\|c\|_1,\quad \mathrm{s.t.}~~c\in [0,1]^n
\end{align*}
Hence problem \eqref{eq9-1} reduces to the standard form in \eqref{eq1-1} with $f(c)=\frac{1}{2}\|A(c)^{-1}\diag(c)u-u\|^2$ and $\varphi(c)=\lambda\|c\|_1$. The gradient of $f$ is given by~\cite[Lemma 5.2]{ochs2014ipiano}
\begin{align}
\label{eq9-2}
 \nabla f(c)=\diag(-Lx+u-x)[A(c)^{\top}]^{-1}(x-u)\quad \text{where} \quad x=A(c)^{-1}\diag(c)u 
\end{align}

Since the Lipschitz constant of $\nabla f$ can not be computed exactly, we use an adaptive $L$ strategy. First, we choose an initial $L_0$. Then in the trial step, we compute $c_{k+1}=\prox{z_k+s_k}$ and let $$L_k=\max\left(2\frac{f(c_{k+1})-f(c_k)-\langle \nabla f(c_k),c_{k+1}-c_k\rangle}{\|c_{k+1}-c_k\|^2},2L_{k-1}\right)$$
We then set $\Lambda=L_k I$ and adjust $\nu,\tau$ accordingly as specified in Section \ref{sec:parameter}. For all the examples used in the subsection, $L_0$ is set to be $0.1$.

The proximal operator is slightly different to the one in subsection~\ref{sec:logistic}. According to~\cite[Theorem 1]{yu2013decomposing}, we know that
\[  \prox{z}=\mathrm{prox}_{[0,1]^n}\circ\mathrm{prox}_{\mu/\lambda \|\cdot\|_1}(z)=\min\{0,\max\{1,\mathrm{prox}_{\mu/\lambda \|\cdot\|_1}(z)\}\}       \]
where the explicit form of $\mathrm{prox}_{\mu \|\cdot\|_1}(z)$ can be found in \eqref{eq:l1prox} and the operations are understood componentwisely. The generalized Jacobian matrix of $\oprox$ is similar to \eqref{eq:generalizedjac}, and can be written as follows by \cite[Example 4.2.17]{milzarek2016numerical}:
\begin{align*}
D_{ii}(z)=\left\{
\begin{aligned}
&0 &  \mathrm{if }z_i\leq \frac{\mu}{\lambda} ~~&\mathrm{ or }~~ z_i\geq \frac{\mu}{\lambda}+1  \\
&1 &  & \mathrm{else}
\end{aligned}
\right.
\end{align*}

Since this problem is nonconvex, most of the algorithms in Section \ref{sec:logistic} are no longer directly applicable here. We compare our algorithm with the following two algorithms:
\begin{itemize}
\item ForBES~\cite{stella2017forward}. We use the same source code as in subsection~\ref{sec:logistic}. Unfortunately, in their setting, $f$ is assumed to be defined all over $\Rn$ which is not the case for \eqref{eq9-1}. To apply ForBES for \eqref{eq9-1}, we use two strategies. The first one, referred as ForBES S1, is to define $f$ to be $\infty$ outside the domain of $c$. Another one, referred as ForBES S2, is to compute $\nabla f$ using \eqref{eq9-2} regardless of whether $c\in[0,1]^n$.  However, both strategies cost too much time to converge to a reasonable solution. For ForBES S1, the line-search strategy would always reach the maximal iteration, because when $x_k^i$, the $i$-th component of $x_k$, is exactly $0$ and the corresponding component of descent direction $d_k$ is negative, then the line-search step in \cite{stella2017forward} would stagnate at this point. The case where $x_k^i$ is $1$ and the corresponding component of $d_k$ is positive is similar. However, this is very likely to happen when the dimension is large. For ForBES S2, what we observe is that, due to the existence of gradient in Forward-backward envelope, it evaluates the gradient at every line-search step, and  the line-search would also requires much more steps to converge because when $x_k$ is near the boundary of $[0,1]^n$ the value of $f$ changes sharply. What we have seen is that ForBES S2 needs about 24 hours to run 2500 iterations for a $512\times 512$ image. Due to these limitations, we didn't report the numerical performance of ForBES.    
\item IPiano~\cite{ochs2014ipiano}. IPiano is an first-order method applying momentum acceleration on forward-backward splitting. We implement this algorithm following the paper. We set $\alpha=\frac{1.99(1-\beta)}{L}$, $\eta=2$ and $\beta =0.8$ as recommended by~\cite{ochs2014ipiano}. The initial Lipschitz constant $L_0$ is set to be $0.1$, too. We also use the trick mentioned in~\cite{ochs2014ipiano}, which means that we increase the Lipschitz constant $L$ by $5\%$ after every 5 steps. 
\end{itemize}
The result of this example was shown in Picture~\ref{fig3} and ~\ref{fig4}.

\begin{figure}[htbp]
\centering
\subfigure[Iteration for books.]{
\includegraphics[width=6cm]{figure/conv_iter_books_512_t1.eps}
}
\quad
\subfigure[Time for books.]{
\includegraphics[width=6cm]{figure/conv_time_books_512_t1.eps}
}
\quad
\subfigure[Iteration for city.]{
\includegraphics[width=6cm]{figure/conv_iter_city_512_t1.eps}
}
\quad
\subfigure[Time for city.]{
\includegraphics[width=6cm]{figure/conv_time_city_512_t1.eps}
}
\quad
 \subfigure[Iteration for coffee.]{
\includegraphics[width=6cm]{figure/conv_iter_coffee_512_t1.eps}
}
\quad
\subfigure[Time for coffee.]{
\includegraphics[width=6cm]{figure/conv_time_coffee_512_t1.eps}
}
\quad
\subfigure[Iteration for mountain.]{
\includegraphics[width=6cm]{figure/conv_iter_mountain_512_t1.eps}
}
\quad
\subfigure[Time for mountain.]{
\includegraphics[width=6cm]{figure/conv_time_mountain_512_t1.eps}
}
%\quad
%\subfigure[pic1. Iteration for stones.]{
%\includegraphics[width=6cm]{figure/conv_iter_stones_512_t1.eps}
%}
%\quad
%\subfigure[pic2. Time for stones.]{
%\includegraphics[width=6cm]{figure/conv_time_stones_512_t1.eps}
%}
\caption{Result for image compression problem. It can be seen that trssn outperforms ipiano for every picture.}
\label{fig3}
\end{figure} 

\begin{figure}[htbp]
\centering
\subfigure[Original figure for books.]{
\includegraphics[width=2.5cm]{figure/books512_t1.png}
}
\subfigure[Mask for books.]{
\includegraphics[width=2.5cm]{figure/mask_trssn_books_512_t1.png}
}
\subfigure[Reconstruction for books.]{
\includegraphics[width=2.5cm]{figure/rec_trssn_books_512_t1.png}
}
\subfigure[Original figure for city.]{
\includegraphics[width=2.5cm]{figure/city512_t1.png}
}
\subfigure[Mask for city.]{
\includegraphics[width=2.5cm]{figure/mask_trssn_city_512_t1.png}
}
\subfigure[Reconstruction for city.]{
\includegraphics[width=2.5cm]{figure/rec_trssn_city_512_t1.png}
}
\subfigure[Original figure for coffee.]{
\includegraphics[width=2.5cm]{figure/coffee512_t1.png}
}
\subfigure[Mask for coffee.]{
\includegraphics[width=2.5cm]{figure/mask_trssn_coffee_512_t1.png}
}
\subfigure[Reconstruction for coffee.]{
\includegraphics[width=2.5cm]{figure/rec_trssn_coffee_512_t1.png}
}
\subfigure[Original figure for mountain.]{
\includegraphics[width=2.5cm]{figure/mountain512_t1.png}
}
\subfigure[Mask for mountain.]{
\includegraphics[width=2.5cm]{figure/mask_trssn_mountain_512_t1.png}
}
\subfigure[Reconstruction for mountain.]{
\includegraphics[width=2.5cm]{figure/rec_trssn_mountain_512_t1.png}
}
\caption{Result of the computed mask and reconstruction figures for the four figures.}
\label{fig4}
\end{figure} 
